Towards More Efficient, Robust, Instance-adaptive, and Generalizable Sequential Decision making

The primary goal of my Ph.D. study is to develop provably efficient and practical algorithms for data-driven sequential decision-making under uncertainty. My work focuses on reinforcement learning (RL), multi-armed bandits, and their applications, including recommendation systems, computer networks, video analytics, and large language models (LLMs). Sequential decision-making methods, such as bandits and RL, have demonstrated remarkable success - ranging from outperforming human players in complex games like Atari and Go to advancing robotics, recommendation systems, and fine-tuning LLMs. Despite these successes, many established algorithms rely on idealized models that can fail under model misspecifications or adversarial perturbations, particularly in settings where accurate prior knowledge of the underlying model class is unavailable or where malicious users operate within dynamic systems. These challenges are pervasive in real-world applications, where robust and adaptive solutions are critical. Furthermore, while worst-case guarantees provide theoretical reliability, they often fail to capture instance-dependent performance, which can lead to more efficient and practical solutions. Another key challenge lies in generalizing to new, unseen environments, a crucial requirement for deploying these methods in dynamic and unpredictable settings. To address these limitations, my research aims to develop more efficient, robust, instance-adaptive, and generalizable sequential decision-making algorithms for both reinforcement learning and bandits. Towards this end, I focus on developing more efficient, robust, instance-adaptive, and generalizable for both general reinforcement learning (RL) and bandits.

==> abstract_in_chinese_2.tex <==
\vspace*{2cm}

\begin{tabular}{lcl}
論文題目 & ： & 更高效、更穩健、具實例自適應性與泛化能力\\
&&的線上學習\\
作者     & ： & 王智勇 \\
學校     & ： & 香港中文大學 \\
學系     & ： & 計算機科學與工程學系 \\
修讀学位 & ： & 哲學博士 \\
摘要     & ： &
\end{tabular}

\vskip 1cm \noindent
我的研究主要目標是設計具理論保證且實用的演算法，用於不確定性下的數據驅動線上序列決策。我專注於強化學習（Reinforcement Learning, RL）、多臂老虎機（Multi-armed Bandits, 多臂老虎機）以及其在推薦系統、電腦網路、影像分析與大型語言模型（Large Language Models, LLMs）等應用領域。線上學習方法（如多臂老虎機與 RL）已在眾多場景中展現驚人成效——從在 Atari 與圍棋等複雜遊戲中超越人類玩家，到推動機器人技術、推薦系統及大型語言模型的精調等應用。

儘管已有這些成功，許多現有演算法仍依賴理想化的模型假設，這些假設在模型錯置（misspecification）或對手擾動下可能失效，特別是在難以獲得正確模型先驗知識的環境或在惡意使用者存在的動態系統中。這些挑戰在真實應用中普遍存在，因此穩健與自適應的解決方案至關重要。此外，儘管最壞情形理論保證具備理論可靠性，但其往往無法反映樣本實例的特徵，從而限制了效率與實用性。另一個關鍵挑戰是如何對新環境進行泛化，這是將這些方法部署於動態與不可預測情境中的必要條件。為解決上述挑戰，我的研究目標是推動該領域邁向：

\begin{center}
\textbf{\textit{更高效、更穩健、具實例自適應性與泛化能力的線上學習}}
\end{center}

因此，我針對強化學習與多臂老虎機兩大類問題，設計具備上述四種性質的演算法。

\noindent\textbf{1. 高效、自適應並具泛化能力的強化學習：}  
強化學習（RL）在從遊戲到自動化系統的多項應用中取得突破性成果。但現階段仍面臨兩大挑戰：一是設計具實例自適應性與高效率的演算法，二是確保這些演算法能有效泛化至新環境。現有 RL 方法多仰賴最壞情形分析，往往過於保守，無法有效利用具體問題的結構特性。此外，許多 RL 演算法在離線設定下難以泛化，導致在測試環境表現不佳。解決這些問題對於推動 RL 理論與實踐至關重要。

我證明，即便是標準的模型式 RL 方法，也能實現無視時間尺度（horizon-free）與變異數相關（variance-dependent）的遺憾界限（regret bound）\cite{wang2024model}。此成果為 RL 理論社群帶來重要貢獻，證明即使是最簡的演算法，在大規模的線上與離線 RL 問題下也能達到緊緻的界限。此外，我也對離線 RL 中的零樣本泛化問題（zero-shot generalization）做出重要貢獻 \cite{wang2024towards}。過去的實證研究指出標準 RL 難以泛化 \cite{mediratta2023generalization}，我首次從理論角度分析此問題，並提出具理論保證且在大型實驗中顯著優於現有方法的解決方案。具體成果如下：

\begin{itemize}
 \item \textbf{簡約方法實現無視時間與次序界限} \cite{wang2024model}：我們首度識別出一種極簡分析框架與演算法，能針對具有函數逼近的一般 RL 問題實現無 horizon 與實例自適應的次序界限（second-order bounds）。無 horizon 意味著界限與 MDP 的時間長度無關，而次序界限會依據策略回報的變異程度縮放，特別當系統近乎確定性或最優策略回報值很小時界限更緊。此成果已被康乃爾大學 CS 6789 課程指定為參考資料。

 \item \textbf{離線強化學習的零樣本泛化} \cite{wang2024towards}：我們研究了離線 RL 中的零樣本泛化（ZSG）問題，代理只從不同環境的資料集中學習，需在未知測試環境中直接執行。我們提出新的架構與理論保證（子最優性差距的上限），並在大型真實資料集（如 Procgen）上顯著優於前人方法。
\end{itemize}

\noindent\textbf{2. 高效、穩健且自適應的多臂老虎機方法：}  
多臂老虎機問題是處理不確定性下序列決策的核心方法，廣泛應用於推薦系統、線上廣告與使用者互動分析等領域。但現有演算法在面對模型錯置、對手擾動與非平穩環境時表現不佳，因此設計穩健且有效的演算法尤為關鍵。

我針對上述問題提出多項具理論保證且兼具實用性的多臂老虎機演算法，特別針對推薦系統的應用。我設計了可處理模型錯置 \cite{wang2024onlinea}、對手破壞 \cite{wang2024onlineb} 及偏好回饋 \cite{wang2025online} 等場景下仍具有效率的演算法，並首度探討動態系統中惡意使用者的即時偵測 \cite{wang2024onlineb}，這是現實中重要但未充分研究的問題。我亦參與了會話式多臂老虎機問題的研究，廣泛應用於交互式推薦系統中 \cite{wang2023efficient, dai2024conversational, dai2024online}。具體成果如下：

\begin{itemize}
 \item \textbf{多臂老虎機聚類的穩健性} \cite{wang2024onlinea}：我們研究了多臂老虎機聚類（Clustering of Bandits, CB）方法，該方法透過使用者偏好間的相似性來提升推薦效果。我們提出能容忍模型錯置與錯誤聚類的穩健演算法，並給出對應理論遺憾上限與實驗驗證。

 \item \textbf{線上惡意使用者偵測} \cite{wang2024onlineb}：面對點擊詐欺、假評論與機器人等行為，我們提出 LOCUD 問題並首次處理雙重目標：一是識別惡意使用者，二是降低決策遺憾。我們提出具理論與實驗保證的通用架構，在推薦系統中同時達到高獎勵與接近離線深度學習方法的偵測精度。

 \item \textbf{會話式多臂老虎機} \cite{wang2023efficient, dai2024conversational, dai2024online}：我們研究會話式多臂老虎機問題，透過詢問使用者關鍵字以加速偏好學習。我們提出 ConLinUCB 架構，整合 arm 與關鍵詞回饋，提出 ConLinUCB-BS 與 ConLinUCB-MCR 等方法，在學習精度與運算效率上顯著優於現有方法。

 \item \textbf{變異數適應的非平穩多臂老虎機} \cite{wang2024variance}：我們研究非平穩線性多臂老虎機問題，提出能利用獎勵變異特性的演算法，包括 Restarted Weighted$\text{OFUL}^+$ 與 Restarted $\text{SAVE}^+$，在變異總量 $V_K < K$ 的情況下顯著優於前人結果。

 \item \textbf{具偏好回饋的多臂老虎機聚類} \cite{wang2025online}：我們首度研究具偏好回饋的多臂老虎機聚類，提出 COLDB（線性偏好）與 CONDB（神經網路偏好）兩大架構，並證明在合作決策下可獲得更小遺憾，並在合成與真實資料集上有顯著實驗成果。

 \item \textbf{其他合作研究} \cite{dai2024quantifying, chu2024online, liu2024combinatorial, yang2024federated, zuo2023adversarial}：我也參與多個應用場景的多臂老虎機研究，包括電腦網路擁塞控制 \cite{dai2024quantifying}、組合多臂老虎機理論 \cite{liu2024combinatorial}、聯邦式多臂老虎機推薦 \cite{yang2024federated} 與安全性分析 \cite{zuo2023adversarial}，擴展了線上學習方法的應用廣度。
\end{itemize}

